Active Inference for Physical AI Agents -- An Engineering Perspective

Physical AI agents, such as robots and other embodied systems operating under tight and fluctuating resource constraints, remain far less capable than biological agents in open-ended real-world environments. This paper argues that Active Inference (AIF), grounded in the Free Energy Principle, offers a principled foundation for closing that gap. We develop this argument from first principles, following a chain from probability theory through Bayesian machine learning and variational inference to active inference and reactive message passing. From the FEP perspective, systems that maintain their structural and functional integrity over time can, under suitable assumptions, be described as minimizing variational free energy (VFE), and AIF operationalizes this by unifying perception, learning, planning, and control within a single computational objective. We show that VFE minimization is naturally realized by reactive message passing on factor graphs, where inference emerges from local, parallel computations. This realization is well matched to the constraints of physical operation, including hard deadlines, asynchronous data, fluctuating power budgets, and changing environments. Because reactive message passing is event-driven, interruptible, and locally adaptable, performance degrades gracefully under reduced resources while model structure can adjust online. We further show that, under suitable coupling and coarse-graining conditions, coupled AIF agents can be described as higher-level AIF agents, yielding a homogeneous architecture based on the same message-passing primitive across scales. Our contribution is not empirical benchmarking, but a clear theoretical and architectural case for the engineering community.

==> examples/unused/exa-efe-football.tex <==
\begin{examplebox}[label=ex:efe-football]{EFE-Based Policy Selection for a Football Player}

A player with the ball must choose between two one-step policies: \emph{shoot} ($u_s$) or \emph{pass} ($u_p$). The relevant future state is $x \in \{1, 0\}$, where $x{=}1$ denotes a scoring opportunity and $x{=}0$ a turnover. The player observes an outcome $y \in \{+, -\}$ after acting.

\smallskip
\textbf{Generative model.}
Following~\eqref{eq:generative-model-for-planning}, the player's generative model for planning consists of a predictive model and a preference model. The \emph{predictive model} $p'(y,x,u) = p'(y|x,u)\,p'(x|u)\,p'(u)$ specifies, for each policy $u$, how future states and observations are expected to unfold. This includes a state prediction $p'(x|u)$ (e.g., the probability of a scoring opportunity given the chosen action) and an observation model $p'(y|x,u)$ (e.g., how reliably the observed outcome reveals the true game state). The \emph{preference model} $\hat{p}(x)$ encodes the player's desired future states. Here, the player strongly prefers scoring opportunities:
\begin{equation*}
    \hat{p}(x{=}1) = 0.9\,,\quad \hat{p}(x{=}0) = 0.1\,.
\end{equation*}
The predicted state beliefs $q(x|u)$ and predicted observation beliefs $q(y|x,u)$ follow from inference under the predictive model $p'$. The EFE~\eqref{eq:Gu-def} then decomposes as
\begin{equation*}
    G(u)
    = \underbrace{\mathrm{KL}\!\left[q(x|u)\,\|\,\hat{p}(x)\right]}_{\text{risk}}
    + \underbrace{\mathbb{E}_{q(x|u)}\!\left[\mathbb{H}\!\left[q(y|x,u)\right]\right]}_{\text{ambiguity}}\,,
\end{equation*}
and the posterior over policies follows from~\eqref{eq:EFE-policy-posterior} (ignoring complexity and policy prior for simplicity):
\begin{equation*}
    q^*(u) = \sigma\!\big({-}G(u)\big)
    = \frac{\exp\!\big({-}G(u)\big)}{\sum_{u'}\exp\!\big({-}G(u')\big)}\,.
\end{equation*}
We consider two scenarios that isolate each component of the EFE.

\medskip
\textbf{Scenario~A: Goal-directed behavior.}
The player believes that passing to a well-positioned teammate has a much higher success rate than shooting, while both policies produce equally informative observations:
\begin{equation*}
\renewcommand{\arraystretch}{1.1}
\begin{array}{l@{\quad}cc@{\qquad}cc}
\toprule
 & q(x{=}1|u) & q(x{=}0|u) & q(+|x{=}1,u) & q(+|x{=}0,u) \\
\midrule
\text{shoot } (u_s) & 0.3 & 0.7 & 0.9 & 0.1 \\
\text{pass } (u_p) & 0.8 & 0.2 & 0.9 & 0.1 \\
\bottomrule
\end{array}
\end{equation*}
Since the observation model is identical for both policies, the ambiguity is the same:
\begin{equation*}
    \text{ambiguity}(u_s) = \text{ambiguity}(u_p)
    = 0.3 \times 0.33 + 0.7 \times 0.33 = 0.33 \;\text{nats}\,.
\end{equation*}
The decision is therefore driven entirely by risk:
\begin{equation*}
\renewcommand{\arraystretch}{1.1}
\begin{array}{l@{\quad}ccc@{\quad}c}
\toprule
 & \text{risk} & \text{ambiguity} & G(u) & q^*(u) \\
\midrule
\text{shoot} & 1.03 & 0.33 & 1.36 & 0.27 \\
\text{pass}  & 0.04 & 0.33 & 0.37 & \mathbf{0.73} \\
\bottomrule
\end{array}
\end{equation*}
Passing is strongly preferred ($73\%$) because it leads to predicted future states closer to the player's preferences. This is \emph{goal-directed} behavior: the player exploits its knowledge that the teammate is well-positioned.

\medskip
\textbf{Scenario~B: Information-seeking behavior.}
Now both policies predict the same success rate, but the observation models differ. Shooting yields uninformative feedback (the outcome depends on goalkeeper reactions that do not reveal the overall game state), whereas passing produces diagnostic observations (a successful pass clearly indicates the game state):
\begin{equation*}
\renewcommand{\arraystretch}{1.1}
\begin{array}{l@{\quad}cc@{\qquad}cc}
\toprule
 & q(x{=}1|u) & q(x{=}0|u) & q(+|x{=}1,u) & q(+|x{=}0,u) \\
\midrule
\text{shoot } (u_s) & 0.5 & 0.5 & 0.6 & 0.4 \\
\text{pass } (u_p) & 0.5 & 0.5 & 0.9 & 0.1 \\
\bottomrule
\end{array}
\end{equation*}
Since the predicted state distributions are identical, the risk is the same:
\begin{equation*}
    \text{risk}(u_s) = \text{risk}(u_p)
    = \mathrm{KL}\!\left[(0.5,\, 0.5)\,\|\,(0.9,\, 0.1)\right] = 0.51 \;\text{nats}\,.
\end{equation*}
The decision is now driven entirely by ambiguity:
\begin{equation*}
\renewcommand{\arraystretch}{1.1}
\begin{array}{l@{\quad}ccc@{\quad}c}
\toprule
 & \text{risk} & \text{ambiguity} & G(u) & q^*(u) \\
\midrule
\text{shoot} & 0.51 & 0.67 & 1.18 & 0.41 \\
\text{pass}  & 0.51 & 0.33 & 0.84 & \mathbf{0.59} \\
\bottomrule
\end{array}
\end{equation*}
Passing is preferred ($59\%$) because it generates observations that are more informative about the game state, even though both policies predict the same success rate. This is \emph{information-seeking} behavior: the player actively gathers information that will improve future decisions.

\medskip
In both scenarios, the EFE automatically selects the preferred policy through a single computation. Scenario~A illustrates exploitation (goal-directed behavior via the risk term), and Scenario~B illustrates exploration (information-seeking behavior via the ambiguity term). In realistic settings with higher-dimensional state spaces, this trade-off is typically richer: a player may sacrifice short-term goal alignment to gather critical information, for example repositioning to observe an occluded part of the pitch before committing to a goal-directed action.

\end{examplebox}


==> examples/unused/exa-vi-denoising-nonlinear.tex <==
\begin{figure}[t]
\begin{tcolorbox}[
    title=Example: Variational Inference for Signal Denoising with a Nonlinear Sensor,
    colback=blue!5!white,
    colframe=blue!40!gray,
    fonttitle=\bfseries]

\textbf{Step 1 — Model.} Consider the state-space model
\begin{align}
    p(x_{1:T},y_{1:T}) &=
    p(x_1)\prod_{t=2}^{T} p(x_t|x_{t-1}) \prod_{t=1}^{T} p(y_t|x_t)\,, \label{eq:nonlinear-denoising-joint-model} \\
    p(x_1) &= \mathcal{N}(x_1|0,\tau^2)\,, \notag\\
    p(x_t|x_{t-1}) &= \mathcal{N}(x_t|x_{t-1},\rho^2)\,, \qquad t=2,\ldots,T\,, \notag\\
    p(y_t|x_t) &= \mathcal{N}(y_t|\tanh(x_t),\sigma^2)\,, \qquad t=1,\ldots,T\,. \notag
\end{align}
The latent state $x_t$ is the clean signal at time $t$, while $y_t$ is a noisy measurement obtained through a saturating nonlinear sensor.

\smallskip
\textbf{Step 2 — Why VI is needed.} The posterior
\[
    p(x_{1:T}|y_{1:T}) = \frac{p(x_{1:T},y_{1:T})}{p(y_{1:T})}
\]
is no longer Gaussian because the observation model depends nonlinearly on $x_t$ through $\tanh(x_t)$. As a result, exact Bayesian inference generally requires intractable high-dimensional integration. Variational inference replaces this by optimization of
\begin{equation}
    F[q] = \int q(x_{1:T})\log\frac{q(x_{1:T})}{p(x_{1:T},y_{1:T})}\,\mathrm{d}x_{1:T}\,.
    \label{eq:nonlinear-denoising-vfe}
\end{equation}

\smallskip
\textbf{Step 3 — Gaussian variational approximation.} Choose
\begin{equation}
    q(x_{1:T}) = \mathcal{N}(x_{1:T}|m,S)\,.
\end{equation}
Substituting the model into \eqref{eq:nonlinear-denoising-vfe} gives
\begin{align}
    F(m,S) &= -\frac{1}{2}\log|S|
    + \frac{1}{2}\,\mathbb{E}_q\!\left[x^\top \Lambda_x x\right]
    + \frac{1}{2\sigma^2}\sum_{t=1}^{T}\mathbb{E}_q\!\left[(y_t-\tanh(x_t))^2\right]
    + \mathrm{const.} \notag\\
    &= -\frac{1}{2}\log|S|
    + \frac{1}{2} m^\top \Lambda_x m
    + \frac{1}{2}\mathrm{tr}(\Lambda_x S)
    + \frac{1}{2\sigma^2}\sum_{t=1}^{T}\mathbb{E}_q\!\left[(y_t-\tanh(x_t))^2\right]
    + \mathrm{const.}
    \label{eq:nonlinear-denoising-vfe-ms}
\end{align}
where $\Lambda_x$ is the tridiagonal prior precision matrix induced by the latent Markov chain. The first three terms are analytic, but the expectation through $\tanh(x_t)$ is not generally available in closed form. In practice, one evaluates or approximates it by local linearization, cubature, quadrature, or Monte Carlo. Minimizing \eqref{eq:nonlinear-denoising-vfe-ms} yields an approximate posterior mean $m_t$ and uncertainty covariance $S$.

\smallskip
\centering
\begin{tikzpicture}[x=0.95cm,y=0.8cm]
\begin{scope}[shift={(0,0)}]
    \draw[->,thin] (0,0) -- (5.2,0) node[right] {$t$};
    \draw[->,thin] (0,-1.6) -- (0,1.8) node[above] {amplitude};
    \draw[gray!50] (0,-1.5) rectangle (5,1.6);
    \node[font=\small\bfseries] at (2.5,1.95) {nonlinear observation model};
    \draw[thick]
        plot[smooth] coordinates {
        (0.0,0.15) (0.4,0.55) (0.8,0.95) (1.2,0.75) (1.6,0.10)
        (2.0,-0.55) (2.4,-0.90) (2.8,-0.45) (3.2,0.20) (3.6,0.85)
        (4.0,1.05) (4.4,0.55) (4.8,-0.10)
        };
    \draw[densely dashed, thick]
        plot[smooth] coordinates {
        (0.0,0.18) (0.4,0.46) (0.8,0.92) (1.2,0.71) (1.6,0.02)
        (2.0,-0.44) (2.4,-0.73) (2.8,-0.40) (3.2,0.16) (3.6,0.68)
        (4.0,0.95) (4.4,0.50) (4.8,-0.03)
        };
    \node[anchor=west,font=\scriptsize] at (3.65,1.05) {$x(t)$};
    \node[anchor=west,font=\scriptsize] at (3.55,0.30) {$y(t)$};
\end{scope}
\begin{scope}[shift={(6.7,0)}]
    \draw[->,thin] (0,0) -- (5.2,0) node[right] {$t$};
    \draw[->,thin] (0,-1.6) -- (0,1.8) node[above] {amplitude};
    \draw[gray!50] (0,-1.5) rectangle (5,1.6);
    \node[font=\small\bfseries] at (2.5,1.95) {variational reconstruction};
    \draw[gray,thin]
        plot[smooth] coordinates {
        (0.0,0.38) (0.4,0.72) (0.8,1.10) (1.2,0.92) (1.6,0.28)
        (2.0,-0.35) (2.4,-0.68) (2.8,-0.28) (3.2,0.38) (3.6,0.98)
        (4.0,1.18) (4.4,0.72) (4.8,0.12)
        };
    \draw[gray,thin]
        plot[smooth] coordinates {
        (0.0,-0.02) (0.4,0.32) (0.8,0.70) (1.2,0.52) (1.6,-0.12)
        (2.0,-0.75) (2.4,-1.08) (2.8,-0.68) (3.2,-0.02) (3.6,0.58)
        (4.0,0.78) (4.4,0.32) (4.8,-0.28)
        };
    \draw[thick]
        plot[smooth] coordinates {
        (0.0,0.18) (0.4,0.52) (0.8,0.90) (1.2,0.72) (1.6,0.08)
        (2.0,-0.55) (2.4,-0.88) (2.8,-0.48) (3.2,0.18) (3.6,0.78)
        (4.0,0.98) (4.4,0.52) (4.8,-0.08)
        };
    \draw[densely dashed, thick]
        plot[smooth] coordinates {
        (0.0,0.18) (0.4,0.46) (0.8,0.92) (1.2,0.71) (1.6,0.02)
        (2.0,-0.44) (2.4,-0.73) (2.8,-0.40) (3.2,0.16) (3.6,0.68)
        (4.0,0.95) (4.4,0.50) (4.8,-0.03)
        };
    \node[anchor=west,font=\scriptsize] at (3.65,0.95) {$m(t)$};
    \node[anchor=west,font=\scriptsize] at (3.55,0.28) {$y(t)$};
    \node[anchor=west,font=\scriptsize] at (3.15,-1.00) {$\pm$ uncertainty};
\end{scope}
\end{tikzpicture}

\end{tcolorbox}
\caption{Variational inference for signal denoising with a nonlinear observation model. Left: the clean latent signal $x_t$ is observed through a saturating nonlinear sensor $y_t \approx \tanh(x_t)$ with additive noise. Right: minimizing the VFE in \eqref{eq:nonlinear-denoising-vfe-ms} over a Gaussian variational posterior yields an approximate reconstruction through the posterior mean $m_t$ and uncertainty covariance $S$.}
\label{fig:vi-denoising-nonlinear}
\end{figure}


==> examples/unused/exa-vi-denoising.tex <==
\begin{figure}[t]
\begin{tcolorbox}[
    title=Example: Variational Inference for Signal Denoising,
    colback=blue!5!white,
    colframe=blue!40!gray,
    fonttitle=\bfseries]

\textbf{Dataset.} We observe a noisy sequence $y=(y_1,\ldots,y_T)^\top \in \mathbb{R}^T$. The task is to retrieve the underlying source signal.

\smallskip  
\textbf{Step 1 — Model.} We use the state-space model
\begin{subequations}\label{eq:denoising-joint-model}
\begin{align}
    p(x_1) &= \mathcal{N}(x_1|0,\tau^2)\,, \notag\\
    p(x_t|x_{t-1}) &= \mathcal{N}(x_t|x_{t-1},\rho^2)\,, \qquad t=2,\ldots,T\,, \notag\\
    p(y_t|x_t) &= \mathcal{N}(y_t|x_t,\sigma^2)\,, \qquad t=1,\ldots,T\,. \notag
\end{align}
\end{subequations}

\smallskip
\textbf{Step 2 — VFE.} Let $x=(x_1,\ldots,x_T)^\top$. The posterior of interest is
$p(x|y) = p(x,y) / p(y)$, but direct Bayesian inference requires the evidence $p(y)$, which may be difficult to evaluate. Variational inference replaces this computation by optimization: choose a tractable approximation $q(x)$ and minimize
\begin{equation}
    F[q] = \int q(x)\log\frac{q(x)}{p(x,y)}\,\mathrm{d}x
         = \underbrace{\mathrm{KL}\!\left[q(x)\,\big\|\,p(x | y)\right]}_{\geq\,0}
           -\,\log p(y)\,.
    \label{eq:denoising-vfe}
\end{equation}
Hence minimizing $F[q]$ drives $q(x)$ toward the posterior while upper-bounding the surprisal.

\smallskip
\textbf{Step 3 — Worked-out objective.} Restrict the variational family to
\begin{equation}
    q(x) = \mathcal{N}(x|m,S)\,.
\end{equation}
Let $\Lambda_x$ denote the tri-diagonal prior precision matrix induced by the Markov chain in \eqref{eq:denoising-joint-model}. Substituting the Gaussian $q$ and the model into \eqref{eq:denoising-vfe} gives
\begin{equation}
    F(m,S) =
    \frac{1}{2} m^\top\!\left(\Lambda_x + \sigma^{-2}I\right)m
    - \sigma^{-2} y^\top m
    + \frac{1}{2}\mathrm{tr}\!\left[\left(\Lambda_x + \sigma^{-2}I\right)S\right]
    - \frac{1}{2}\log|S|
    + \mathrm{const.}
    \label{eq:denoising-vfe-ms}
\end{equation}
Thus, VI reduces to an optimization problem over the mean vector $m$ and covariance matrix $S$. The posterior mean $m_t$ yields the denoised signal estimate, while the diagonal entries of $S$ quantify uncertainty (right panel below).

\smallskip
\centering
\begin{tikzpicture}[x=0.95cm,y=0.8cm]
\begin{scope}[shift={(0,0)}]
    \draw[->,thin] (0,0) -- (5.2,0) node[right] {$t$};
    \draw[->,thin] (0,-1.6) -- (0,1.8) node[above] {amplitude};
    \draw[gray!50] (0,-1.5) rectangle (5,1.6);
    \node[font=\small\bfseries] at (2.5,1.95) {observation model};
    \draw[thick]
        plot[smooth] coordinates {
        (0.0,0.15) (0.4,0.55) (0.8,0.95) (1.2,0.75) (1.6,0.10)
        (2.0,-0.55) (2.4,-0.90) (2.8,-0.45) (3.2,0.20) (3.6,0.85)
        (4.0,1.05) (4.4,0.55) (4.8,-0.10)
        };
    \draw[densely dashed, thick]
        plot[smooth] coordinates {
        (0.0,0.35) (0.4,0.15) (0.8,1.20) (1.2,0.45) (1.6,0.45)
        (2.0,-0.95) (2.4,-0.45) (2.8,-0.85) (3.2,0.55) (3.6,0.55)
        (4.0,1.30) (4.4,0.20) (4.8,0.15)
        };
    \node[anchor=west,font=\scriptsize] at (3.65,1.05) {$x(t)$};
    \node[anchor=west,font=\scriptsize] at (3.55,0.35) {$y(t)$};
\end{scope}
\begin{scope}[shift={(6.7,0)}]
    \draw[->,thin] (0,0) -- (5.2,0) node[right] {$t$};
    \draw[->,thin] (0,-1.6) -- (0,1.8) node[above] {amplitude};
    \draw[gray!50] (0,-1.5) rectangle (5,1.6);
    \node[font=\small\bfseries] at (2.5,1.95) {variational reconstruction};
    \draw[gray,thin]
        plot[smooth] coordinates {
        (0.0,0.38) (0.4,0.72) (0.8,1.10) (1.2,0.92) (1.6,0.28)
        (2.0,-0.35) (2.4,-0.68) (2.8,-0.28) (3.2,0.38) (3.6,0.98)
        (4.0,1.18) (4.4,0.72) (4.8,0.12)
        };
    \draw[gray,thin]
        plot[smooth] coordinates {
        (0.0,-0.02) (0.4,0.32) (0.8,0.70) (1.2,0.52) (1.6,-0.12)
        (2.0,-0.75) (2.4,-1.08) (2.8,-0.68) (3.2,-0.02) (3.6,0.58)
        (4.0,0.78) (4.4,0.32) (4.8,-0.28)
        };
    \draw[thick]
        plot[smooth] coordinates {
        (0.0,0.18) (0.4,0.52) (0.8,0.90) (1.2,0.72) (1.6,0.08)
        (2.0,-0.55) (2.4,-0.88) (2.8,-0.48) (3.2,0.18) (3.6,0.78)
        (4.0,0.98) (4.4,0.52) (4.8,-0.08)
        };
    \draw[densely dashed, thick]
        plot[smooth] coordinates {
        (0.0,0.35) (0.4,0.15) (0.8,1.20) (1.2,0.45) (1.6,0.45)
        (2.0,-0.95) (2.4,-0.45) (2.8,-0.85) (3.2,0.55) (3.6,0.55)
        (4.0,1.30) (4.4,0.20) (4.8,0.15)
        };
    \node[anchor=west,font=\scriptsize] at (3.65,0.95) {$m(t)$};
    \node[anchor=west,font=\scriptsize] at (3.55,0.30) {$y(t)$};
    \node[anchor=west,font=\scriptsize] at (3.15,-1.00) {$\pm$ uncertainty};
\end{scope}
\end{tikzpicture}

\end{tcolorbox}
\caption{Variational inference for time-series denoising. Left: a latent signal $x_t$ evolves smoothly over time and generates noisy observations $y_t$. Right: minimizing \eqref{eq:denoising-vfe-ms} over the Gaussian variational parameters $(m,S)$ yields a denoised trajectory through the posterior mean $m_t$ and uncertainty bands through the posterior covariance $S$.}
\label{fig:vi-denoising}
\end{figure}


==> figures/unused/fig-player-fg.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
    factor/.style={rectangle, draw, fill=black!15, minimum size=7mm, inner sep=1pt, font=\small},
    eqnode/.style={rectangle, draw, fill=white, minimum size=4mm, inner sep=0pt, font=\scriptsize},
    edge label/.style={font=\small, midway},
    halfedge/.style={-},
    >=Stealth,
    node distance=1.8cm,
]

% ---- Main horizontal chain ----

% Prior on current state (from perception)
\node[factor] (f0) at (0, 0) {$\delta_{\hat{x}_0}$};

% Transition factors
\node[factor] (ft1) at (2.8, 0) {$f_{\mathrm{t}}$};
\node[factor] (ft2) at (7.2, 0) {$f_{\mathrm{t}}$};

% Equality nodes (branch x_1 and x_2 to multiple factors)
\node[eqnode] (eq1) at (5.0, 0) {$=$};
\node[eqnode] (eq2) at (9.4, 0) {$=$};

% Main chain edges
\draw[thick] (f0)  -- node[above, font=\small] {$\hat{x}_0$} (ft1);
\draw[thick] (ft1) -- node[above, font=\small] {$x_1$} (eq1);
\draw[thick] (eq1) -- (ft2);
\draw[thick] (ft2) -- node[above, font=\small] {$x_2$} (eq2);

% ---- Observation model (above) ----

\node[factor] (fo1) at (5.0, 1.8) {$f_{\mathrm{o}}$};
\node[factor] (fo2) at (9.4, 1.8) {$f_{\mathrm{o}}$};

\draw[thick] (eq1) -- (fo1);
\draw[thick] (eq2) -- (fo2);

% Predicted observations (half-edges)
\draw[thick] (fo1) -- +(0, 1.0) node[above, font=\small] {$y_1$};
\draw[thick] (fo2) -- +(0, 1.0) node[above, font=\small] {$y_2$};

% ---- Preference + epistemic priors on states (below eq nodes) ----

\node[factor] (fpx1) at (5.0, -1.6) {$\hat{f}_x$};
\node[factor] (fpx2) at (9.4, -1.6) {$\hat{f}_x$};

\draw[thick] (eq1) -- (fpx1);
\draw[thick] (eq2) -- (fpx2);

% ---- Control variables and policy priors (below transition factors) ----

\node[factor] (fpu1) at (2.8, -1.6) {$\tilde{f}_u$};
\node[factor] (fpu2) at (7.2, -1.6) {$\tilde{f}_u$};

\draw[thick] (ft1) -- node[right, font=\small] {$u_1$} (fpu1);
\draw[thick] (ft2) -- node[right, font=\small] {$u_2$} (fpu2);

% ---- Time annotation ----
\draw[thin, gray, ->] (0, -2.8) -- (10.2, -2.8) node[right, font=\small, gray] {planning horizon};
\node[font=\scriptsize, gray, below] at (0, -2.8) {$t$};
\node[font=\scriptsize, gray, below] at (5.0, -2.8) {$t{+}1$};
\node[font=\scriptsize, gray, below] at (9.4, -2.8) {$t{+}2$};

% ---- Annotations (right side) ----
\begin{scope}[font=\scriptsize, text width=3.6cm, anchor=west]
    \node[right] at (10.6, 1.8)  {$f_{\mathrm{o}}(y_t, x_t) = p'(y_t | x_t)$\\[1pt] observation model\\(camera, lidar, proprioception)};
    \node[right] at (10.6, 0)    {$f_{\mathrm{t}}(x_t, u_t, x_{t+1}) = p'(x_{t+1} | x_t, u_t)$\\[1pt] state transition\\(game dynamics)};
    \node[right] at (10.6, -1.6) {$\hat{f}_x(x_t) = \hat{p}(x_t)\tilde{p}(x_t)$\\[1pt] preference $+$ epistemic prior\\(scoring position, visibility)};
\end{scope}

\begin{scope}[font=\scriptsize, text width=3.2cm, anchor=east]
    \node[left] at (-0.8, -1.6) {$\tilde{f}_u(u_t) = p'(u_t)\tilde{p}(u_t)$\\[1pt] policy prior $+$ epistemic\\(habitual plays, flexibility)};
    \node[left] at (-0.8, 0) {$\delta_{\hat{x}_0}$: current state\\estimate from perception\\(ball, teammates, opponents)};
\end{scope}

\end{tikzpicture}
\caption{Forney-style factor graph for a single football player's planning model over a two-step horizon. The current state estimate $\hat{x}_0$ (obtained by perceptual inference) anchors a predictive rollout in which the player evaluates candidate action sequences $(u_1, u_2)$. Equality nodes ($=$) branch each future state $x_t$ to the transition, observation, and prior factors. The factor $\hat{f}_x$ combines preference priors $\hat{p}(x)$ (e.g., reach a scoring position) with epistemic priors $\tilde{p}(x)$ that favor informative future states. The factor $\tilde{f}_u$ combines the empirical policy prior $p'(u)$ with the epistemic prior $\tilde{p}(u)$ that favors flexible action sequences. Minimizing the VFE over this graph yields the posterior $q^*(u)$ of~\eqref{eq:EFE-policy-posterior}, which balances goal-directed and information-seeking behavior.}
\label{fig:player-fg}
\end{figure}


==> figures/unused/tab-notation.tex <==
\begin{table}[h!]
\centering
\small
\caption{Summary of principal notation.}
\label{tab:notation}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Symbol} & \textbf{Description} \\
\midrule
\multicolumn{2}{@{}l}{\emph{Agent state partition}} \\
$y$ & Sensory (observation) states \\
$x$ & External (environmental) states \\
$u$ & Control (active) states; a policy is a sequence of $u$ \\
$s$ & Internal (agent) states \\
$\alpha = (s, u)$ & Autonomous states \\
\midrule
\multicolumn{2}{@{}l}{\emph{Probability densities}} \\
$p(\cdot)$ & Model-defined or steady-state density \\
$p'(\cdot)$ & Predictive model for future dynamics \\
$\hat{p}(x)$ & Preference prior over future states \\
$\tilde{p}(x),\;\tilde{p}(u)$ & Epistemic priors \\
$f(y,x,u)$ & Generative model for planning \\
$q(\cdot)$ & Variational (approximate) posterior \\
\midrule
\multicolumn{2}{@{}l}{\emph{Functionals and cost terms}} \\
$F[q]$ & Variational Free Energy (VFE) \\
$G(u)$ & Expected Free Energy (EFE) \\
$C(u)$ & Complexity cost for policy $u$ \\
$P(u)$ & Empirical policy prior cost \\
$S[q]$ & Relative entropy ($= -F[q]$) \\
\midrule
\multicolumn{2}{@{}l}{\emph{Other}} \\
$D$ & Observed data set \\
$\theta$ & Model parameters \\
$\mathrm{KL}[q \| p]$ & Kullback--Leibler divergence \\
$\mathbb{H}[q]$ & Shannon entropy of $q$ \\
$\sigma(\cdot)$ & Softmax function \\
\bottomrule
\end{tabular}
\end{table}


==> sections/unused/aif-example.tex <==
\section{Example: Two Coupled Thermostat Agents}\label{sec:thermostat-example}

To make the three conditions concrete, consider two rooms in a building, each equipped with a thermostat implemented as an AIF agent. The rooms are thermally coupled through a shared wall.

\subsection*{Individual agents}
Agent $A$ holds a generative model
\begin{equation}
p(y_A|x_A) = \mathcal{N}(y_A | x, \sigma_y^2)\,, \qquad p(x_A) = \mathcal{N}(x_A | \hat{x}, \sigma_x^2)
\end{equation}
where $y_A$ and $x_A$ are the observed and true (unknown) temperatures in room~1, respectively. Agent $A$ maintains a belief $q_A(x_A) = \mathcal{N}(x_A | \mu_A, v_A)$ about the true temperature  in room~1 and its VFE is (see Appendix~\ref{app:thermostat-vfe} for derivation)
\begin{subequations}\label{eq:thermostat-vfe-a}
    \begin{align}
    F_A[q_A] &=  F_A(\mu_A, v_A) = \mathbb{E}_{q_A}\left[\log\frac{q_A(x_A)}{p(y_A,\,x_A)}\right] \\
    &= \frac{(\mu_A - \hat{x})^2 + v_A}{2\sigma_x^2}
    + \frac{(y_A - \mu_A)^2 + v_A}{2\sigma_y^2}
    - \tfrac{1}{2}\ln v_A + \mathrm{const.}
    \end{align}
\end{subequations}

Minimizing \eqref{eq:thermostat-vfe-a} over internal states $s_A = (\mu_A,v_A)$ yields the standard Bayesian (Kalman) update (derived in Appendix~\ref{app:thermostat-vfe}):
\begin{equation}\label{eq:thermostat-solo}
     \mu_A^* = \frac{\hat{x}/\sigma_x^2 + y_A/\sigma_y^2}{1/\sigma_x^2 + 1/\sigma_y^2}\,, \qquad  \frac{1}{v_A^*} = \frac{1}{\sigma_x^2}+\frac{1}{\sigma_y^2}\,.
\end{equation}
Agent $B$ operates identically in room~2, producing $\mu_B^*$ and $v_B^*$.

With $\sigma_x^2 = 4\,^\circ\mathrm{C}^2$, $\sigma_y^2 = 1\,^\circ\mathrm{C}^2$, $\hat{x} = 20\,^\circ\mathrm{C}$, and observations $y_A = 21\,^\circ\mathrm{C}$, $y_B = 23\,^\circ\mathrm{C}$, the uncoupled posteriors are
\begin{equation}\label{eq:thermostat-solo-nums}
    \mu_A^* = 20.8\,^\circ\mathrm{C}, \quad \mu_B^* = 22.4\,^\circ\mathrm{C}, \quad v_A^* = v_B^* = 0.8\,^\circ\mathrm{C}^2.
\end{equation}

\subsection*{Introduce thermal coupling (E1 in effect)}
The shared wall creates a thermal link between $x_A$ and $x_B$: heat flows across the wall until the temperatures equilibrate, so knowing $x_A$ gives probabilistic information about $x_B$. We model this at thermal steady state as \begin{equation}
    p(x_B | x_A) = \mathcal{N}(x_B | x_A + \delta,\, \sigma_c^2) \,,
\end{equation}
which replaces the previous prior belief $p(x_B) = \mathcal{N}(x_B | \hat{x}, \sigma_x^2)$. The offset $\delta$ is the mean temperature gradient maintained by external boundary conditions (e.g., a stairwell or exterior wall on one side); setting $\delta = 0$ means both rooms tend toward the same equilibrium. The variance $\sigma_c^2$ captures the tightness of the coupling: a perfectly conducting wall gives $\sigma_c^2 \to 0$ (temperatures are locked together), while a perfectly insulating wall gives $\sigma_c^2 \to \infty$ (rooms decouple). With $\sigma_c^2 = 1\,^\circ\mathrm{C}^2$, the wall provides as much information about the adjacent temperature as a direct measurement ($\sigma_y^2 = 1\,^\circ\mathrm{C}^2$), making the coupling strong enough to materially affect each agent's posterior.

Condition E1 is satisfied because the coupling operates \emph{through the environment} (the wall temperature is a shared blanket state), not by directly linking $\mu_A$ to $\mu_B$: . The collective blanket property follows from F3 and E1: $(y_A, a_A, y_B, a_B)$ screens $(\mu_A, \mu_B)$ from the environment outside the building.

\subsection*{Collective VFE}
The joint generative model is now
\begin{equation}
    p(y_A, y_B,x_A, x_B) = p(y_A|x_A)\,p(y_B|x_B)\,\underbrace{p(x_B|x_A)}_{\text{coupling}}\,p(x_A)\,. 
\end{equation}
Under the mean-field approximation $q_C(x_A, x_B) = q_A(x_A)\,q_B(x_B)$ (valid when Condition E2 holds, i.e.\ when local inference is faster than the thermal coupling), the collective VFE (derived in Appendix~\ref{app:thermostat-collective-vfe}) decomposes as
\begin{equation}\label{eq:thermostat-collective-vfe}
    F_C = F_A(\mu_A, v_A) + F_{B|A}(\mu_B, v_B , \mu_A, v_A)\,,
\end{equation}
where $F_{B|A}$ is agent $B$'s VFE for the model $p(y_B|x_B)p(x_B|x_A)$:
\begin{equation}\label{eq:thermostat-vfe-bca}
    F_{B|A}(\mu_B, v_B , \mu_A, v_A)
    = \frac{(y_B - \mu_B)^2 + v_B}{2\sigma_y^2}
    + \underbrace{\frac{(\mu_B - \mu_A - \delta)^2 + v_A + v_B}{2\sigma_c^2}}_{\text{coupling term}}
    - \tfrac{1}{2}\ln v_B + \mathrm{const.}
\end{equation}
Comparing $F_{B|A}$ to the uncoupled $F_B$, the only difference is that the independent prior term $\frac{(\mu_B - \hat{x})^2 + v_B}{2\sigma_x^2}$ is replaced by the coupling term $\frac{(\mu_B - \mu_A - \delta)^2 + v_A + v_B}{2\sigma_c^2}$: the wall pins $x_B$ relative to $x_A$ rather than to the global mean $\hat{x}$. Minimizing \eqref{eq:thermostat-collective-vfe} yields the following optimal beliefs (derived in Appendix~\ref{app:thermostat-coupled-update}):
\begin{alignat}{2}
    \mu_A &= \frac{\hat{x}/\sigma_x^2 + y_A/\sigma_y^2 + (\mu_B - \delta)/\sigma_c^2}{1/\sigma_x^2 + 1/\sigma_y^2 + 1/\sigma_c^2}\,, &\qquad \frac{1}{v_A} &= \frac{1}{\sigma_x^2} + \frac{1}{\sigma_y^2} + \frac{1}{\sigma_c^2}\,, \label{eq:coupled-update-a} \\[4pt]
    \mu_B &= \frac{y_B/\sigma_y^2 + (\mu_A + \delta)/\sigma_c^2}{1/\sigma_y^2 + 1/\sigma_c^2}\,, &\qquad \frac{1}{v_B} &= \frac{1}{\sigma_y^2} + \frac{1}{\sigma_c^2}\,. \label{eq:coupled-update-b}
\end{alignat}
The means in \eqref{eq:coupled-update-a}--\eqref{eq:coupled-update-b} are coupled and solved in closed form by substituting \eqref{eq:coupled-update-b} into \eqref{eq:coupled-update-a}; the variances decouple and follow directly from $\partial F_C/\partial v_i = 0$. With the numerical values above the result is
\begin{equation}\label{eq:thermostat-coupled-nums}
    \mu_A = 21.4\,^\circ\mathrm{C}, \quad \mu_B = 22.2\,^\circ\mathrm{C}, \quad v_A = 0.44\,^\circ\mathrm{C}^2, \quad v_B = 0.50\,^\circ\mathrm{C}^2.
\end{equation}
Two effects are worth noting: 
\begin{itemize}
    \item First, the coupled beliefs are shifted relative to the uncoupled values \eqref{eq:thermostat-solo-nums}: agent $A$'s estimate is pulled up ($20.8 \to 21.4\,^\circ\mathrm{C}$) by the information that the adjacent room is warmer, and agent $B$'s estimate is pulled down ($22.4 \to 22.2\,^\circ\mathrm{C}$) accordingly.
    \item Second, and more fundamentally, the posterior variance of each agent is \emph{reduced} by the coupling: $v_A$ falls from $0.8$ to $0.44\,^\circ\mathrm{C}^2$. The collective is more certain than either agent alone, because the wall provides an additional information source with precision $1/\sigma_c^2 = 1$ that each agent can exploit via the other's measurement. This is the informational advantage of nested AIF: the collective precision is
\begin{equation}\label{eq:collective-precision}
    v_A^{-1} = \sigma_x^{-2} + \sigma_y^{-2} + \sigma_c^{-2} = 0.25 + 1 + 1 = 2.25\,^\circ\mathrm{C}^{-2}\,,
\end{equation}
exceeding the individual precision $v_A^{*-1} = 1.25\,^\circ\mathrm{C}^{-2}$ by a factor of $1.8$.
\end{itemize}

\subsection*{What breaks the nested structure?}

Two failure modes deserve explicit treatment. 
\begin{itemize}
    \item If Condition E1 is violated (for example, if agent $A$'s heater control signal directly enters agent $B$'s belief update, a direct internal-to-internal link bypassing the wall), the coupling term in \eqref{eq:thermostat-collective-vfe} becomes a non-decomposable cross-term in $(\mu_A, \mu_B)$ that cannot be attributed to either agent independently. The mean-field factorization $q_A q_B$ is no longer a valid approximation and the two agents must be treated as a single unpartitioned system with a redesigned Markov blanket.
    \item If Condition E2 is violated (say, the wall is so thin that thermal coupling acts on the same millisecond timescale as each thermostat's measurement cycle), the adiabatic approximation fails. Equations \eqref{eq:coupled-update-a}--\eqref{eq:coupled-update-b} become simultaneous rather than sequentially consistent, and the mean-field approximation introduces errors proportional to the coupling-to-noise ratio $\sigma_y^2/\sigma_c^2$. In the limit $\sigma_c^2 \to 0$ the two rooms are thermally fused and the only valid description is a single agent tracking the common temperature.
\end{itemize}


==> sections/unused/biographies.tex <==
\section{Biographies}
\label{sec:bio}
For long C\&F articles you are asked to include a 100-word biography. Here is the required information:
//Author Name// //(email address)// received his/her //highest degree// in //area// from //institution//. [Do not need to list the year but can use it if it is provided. OK to list location if provided but not required.] He/she is a //role// at //institution, city/state/postal code/country//. //Last name// serves as a //role// on //related publication or Society//. [List 2-3 major awards.] //His/her// research interests include //3-5//. //Last name// is a //IEEE membership level// (if applicable).



==> sections/unused/engineering-walkthrough.tex <==
\section{Active Inference: An Engineering Walkthrough}
\label{sec:engineering-walkthrough}
%---------------------------------------------------------------

The preceding sections established that AIF is VFE minimization, and that collections of AIF agents satisfying mild structural conditions are themselves AIF agents. This section provides a self-contained, engineering-focused walkthrough of these results. We trace the full arc from stochastic dynamics (F1--F3) through variational inference, nested agents, and the emergence of goal-directed and exploratory behavior, to a practical reactive message-passing implementation and a distributed robot football example.

%---------------------------------------------------------------
\subsection{From Stochastic Physics to Autonomous Dynamics}
%---------------------------------------------------------------

The combined state of the agent and its environment is $z = (y, x, u, s)$, where $y$ are sensory (observation) states, $x$ are external (environmental) states, $u$ are control (active) states, and $s$ are internal (autonomous) states. The autonomous states are $\alpha = (u,s)$; the pair $(y,u)$ constitutes the Markov blanket. The FEP rests on three assumptions \cite{fristonlife2013,fristonfree2019,fristonfree2022,fristonpath2023}.

\begin{itemize}
    \item[\textbf{F1}] \textit{Langevin dynamics.}
    The full state evolves according to a stochastic differential equation,
    \begin{equation}\label{eq:eng-langevin}
        \dot{z} = f(z) + \omega\,, \qquad \omega \sim \mathcal{N}(0,\,2\Gamma)\,,
    \end{equation}
    where $f(z)$ is a deterministic flow field and $\Gamma \succeq 0$ is the diffusion matrix.

    \item[\textbf{F2}] \textit{Non-equilibrium steady state.}
    The system converges to a stationary density $p(z) = p(y,x,u,s)$ that remains
    time-invariant while probability continues to circulate through state space. The agent
    thereby occupies a bounded region of state space indefinitely, maintaining its
    structural integrity~\cite{fristonlife2013}.

    \item[\textbf{F3}] \textit{Markov blanket.}
    The pair $(y,u)$ statistically separates internal states $s$ from external states $x$:
    \begin{equation}\label{eq:eng-MB}
        x \;\perp\; s \;\big|\; (y,\,u)\,.
    \end{equation}
    This conditional independence defines the agent as a distinct entity within the larger
    dynamical system.
\end{itemize}

From F1 and F2, the NESS condition ($\nabla \cdot j = 0$ for the probability current $j$) implies a Helmholtz decomposition of the flow field \cite[Eq.~1.8]{fristonfree2019}:
\begin{equation}\label{eq:eng-helmholtz}
    f(z) = \bigl(\Gamma + Q(z)\bigr)\,\nabla\log p(z)\,,
\end{equation}
where $Q = -Q^\top$ is antisymmetric (solenoidal). The dissipative part $\Gamma\,\nabla\log p$ performs gradient ascent on the log-density; the solenoidal part $Q\,\nabla\log p$ circulates probability without altering it.

Restricting \eqref{eq:eng-helmholtz} to the autonomous states $\alpha = (u,s)$ and applying the Markov blanket condition via the marginal flow lemma \cite[Eq.~1.22]{fristonfree2019}:
\begin{equation}\label{eq:eng-grad-split}
    \nabla_\alpha \log p(y,x,u,s) = \underbrace{\nabla_\alpha \log p(x|y,u)}_{\text{absorbed into solenoidal flow}} + \nabla_\alpha \log p(y,u,s)\,.
\end{equation}
The first term on the right does not depend on internal states $s$ (by F3), and its contribution to the dissipative flow can be absorbed into the solenoidal component $Q_{\alpha\alpha}$. The dominant gradient (dissipative) flow of the autonomous states is therefore \cite{fristonlife2013,fristonfree2022}:
\begin{equation}\label{eq:eng-auto-dynamics}
\boxed{\dot{\alpha} = \dot{(u,s)} \;\propto\; \nabla_\alpha \log p(y,\,u,\,s)\,.}
\end{equation}

This is the central mathematical result of the FEP under assumptions F1--F3. Whenever the agent drifts toward regions of low steady-state probability (high surprisal), the gradient flow \eqref{eq:eng-auto-dynamics} pushes it back toward more probable configurations, maintaining its recognizable form over time.

Both internal states $s$ (perception) and control states $u$ (action) are inferred simultaneously from the same gradient. There is no separate control law: actions are inferred, not commanded.

%---------------------------------------------------------------
\subsection{Variational Inference, the Generative Model, and the Gibbs Form}
%---------------------------------------------------------------

Equation \eqref{eq:eng-auto-dynamics} is a statement about the physics of self-organizing systems. Its variational reinterpretation connects it to Bayesian machine learning.

\subsubsection{Recognition density}\label{sec:recognition-density} Because internal states $s$ are shielded from external states $x$ by the Markov blanket (F3), we may interpret $s$ as parameterizing a \emph{recognition density}, a probability distribution over external states $x$, inferred from sensory inputs and control states:
\begin{equation}\label{eq:eng-recognition}
    s \;\mapsto\; q(x|s)\,.
\end{equation}
For example, if $s = (\mu, \sigma^2)$, then $q(x|s) = \mathcal{N}(x|\mu, \sigma^2)$. Under this interpretation, the gradient flow \eqref{eq:eng-auto-dynamics} can be re-expressed as VFE minimization \cite{fristonfree2022,fristonpath2023}:
\begin{equation}\label{eq:eng-vfe}
    F[q_s] = \int q(x|s)\,\log\frac{q(x|s)}{p(y,x,u)}\,\mathrm{d}x = \underbrace{\mathrm{KL}\bigl[q(x|s)\,\|\,p(x|y,u)\bigr]}_{\geq\,0} - \log p(y,u)\,.
\end{equation}

Since the KL divergence is non-negative, $F[q_s]$ is an upper bound on negative log-evidence $-\log p(y,u)$. Global minimization drives $q(x|s) \to p(x|y,u)$ and $F \to -\log p(y,u)$, recovering exact Bayesian inference. The gradient flow \eqref{eq:eng-auto-dynamics} is the physical realization of descending on $F[q_s]$.

\subsubsection{Generative model}\label{sec:eng-generative-model} The joint density $p(y,x,u)$ in \eqref{eq:eng-vfe} is the agent's \emph{generative model}, a probabilistic description of how observations arise from external causes and how controls affect the world. A typical factorization is:
\begin{equation}\label{eq:eng-gen-model}
    p(y,x,u) = \underbrace{p(y|x)}_{\text{sensor model}}\,\underbrace{p(x|u)}_{\text{dynamics model}}\,\underbrace{p(u)}_{\text{control prior}}\,.
\end{equation}
To a signal processing engineer, this is a probabilistic state-space model: $p(y|x)$ is the measurement equation and $p(x|u)$ is the state-transition equation. For linear-Gaussian models, VFE minimization over $q(x|s)$ reproduces the Kalman filter equations.

\subsubsection{Gibbs form}\label{sec:gibbs-form} The posterior over internal states $p(s|y,u)$ takes a Gibbs (Boltzmann) form. From Bayes rule and \eqref{eq:eng-gen-model}:
\begin{equation}\label{eq:eng-gibbs}
    p(s|y,u) \;\propto\; p(y|s)\,p(s) \;\propto\; \exp\bigl(-E(s;\,y,u)\bigr)\,,
\end{equation}
where $E(s;\,y,u) = -\log p(y|s) - \log p(s)$ is the \emph{energy function}. Gradient descent on VFE is equivalent to descending on this energy, a perspective familiar from Hopfield networks and statistical physics. The Gibbs form is also implementation-friendly: the energy $E$ decomposes additively over local factors of the generative model, enabling fully distributed computation.

\textbf{Key insight for the signal processing engineer.} The AIF agent is a real-time Bayesian filter. Its internal states $s$ continuously estimate the external world $x$ via the forward model $p(y|x)$ and the dynamics $p(x|u)$. The key distinction from classical signal processing is that control states $u$ are \emph{inferred} as part of the same gradient flow, not issued as external commands. Perception (updating $s$ to minimize prediction errors on $y$) and control (updating $u$ to bring $y$ closer to predictions) are simultaneous outputs of a single VFE minimization process.

%---------------------------------------------------------------
\subsection{Interacting AIF Agents Form a New AIF Agent}
%---------------------------------------------------------------

A central design question for distributed physical AI is: when does a network of AIF agents behave as a single, higher-level AIF agent? The answer is provided by three conditions \cite{fristonlife2013,fristonparcels2020,fristonfree2019}.

\begin{itemize}
    \item[\textbf{E1}] \textit{Sparse coupling.}
    Internal states $s_i$ of one agent do not directly drive internal states $s_j$ of
    another. All inter-agent influence flows through blanket (sensory or control) states.
    In factor-graph terms, there are no edges between internal-state nodes of different
    agents. F3 and E1 together imply a \emph{collective Markov blanket}:
    $x_\mathrm{env} \perp \{s_i\} \,|\, \{(y_i,u_i)\}$ (two-step d-separation). % chktex 3

    \item[\textbf{E2}] \textit{Timescale separation.}
    Each agent's local inference operates on a faster timescale than inter-agent coupling.
    This adiabatic condition allows each agent to reach its local steady state before the
    coupling reshapes its effective prior. Fast internal fluctuations average out and do
    not propagate between agents.

    \item[\textbf{E3}] \textit{Feedback closure.}
    The collective dynamics must feed back onto the constituent agents so the ensemble
    stabilizes as a coherent self-organizing unit.
\end{itemize}

When E1--E3 hold, the collective VFE retains the same KL-divergence structure as the individual VFEs. No new inference principle is required at the group level.

\subsubsection{Example: two robots tracking a shared object}\label{sec:two-robots-example} Consider two robots $A$ and $B$ that jointly estimate the position $x$ of a moving object, each with its own noisy sensor:
\begin{align*}
    p(y_A|x) &= \mathcal{N}(y_A | x,\,\sigma_A^2)\,, \quad \sigma_A^2 = 1\,; \quad
    p(y_B|x) = \mathcal{N}(y_B | x,\,\sigma_B^2)\,, \quad \sigma_B^2 = 2\,; \quad
    p(x) = \mathcal{N}(x | 0,\,4)\,.
\end{align*}
With observations $y_A = 2$, $y_B = 3$, individual VFE minimization yields Kalman updates:
\begin{align*}
    \mu_A^* &= \tfrac{2/1\;+\;0/4}{1/1\;+\;1/4} = 1.60\,, \quad v_A^* = \tfrac{1}{1.25} = 0.80\,;\\[3pt]
    \mu_B^* &= \tfrac{3/2\;+\;0/4}{1/2\;+\;1/4} = 2.00\,, \quad v_B^* = \tfrac{1}{0.75} = 1.33\,.
\end{align*}
The robots interact through the shared object $x$ (E1), satisfying sparse coupling; the collective blanket property follows from F3 and E1. Their inference cycles are faster than object motion (E2). The collective VFE under the joint model $p(y_A,y_B,x) = p(y_A|x)\,p(y_B|x)\,p(x)$ gives the fused estimate:
\begin{equation}\label{eq:eng-fusion}
    \mu_C^* = \frac{2/1 + 3/2 + 0/4}{1 + 1/2 + 1/4} = \frac{3.5}{1.75} = 2.00\,, \qquad v_C^* = \frac{1}{1.75} = 0.57\,.
\end{equation}
The collective posterior variance ($v_C^* = 0.57$) is smaller than either individual variance ($v_A^* = 0.80$, $v_B^* = 1.33$), because the two sensors provide complementary information. The collective VFE retains the same KL-divergence structure as the individual VFEs, confirming that the pair $\{A,B\}$ is itself an AIF agent. A third robot can couple to $\{A,B\}$ at a higher level, creating a hierarchy with no new principle required at any scale.

%---------------------------------------------------------------
\subsection{Precise Agents and the Emergence of Expected Free Energy}
%---------------------------------------------------------------

Equation \eqref{eq:eng-auto-dynamics} governs perceptual inference: internal states $s$ track the external environment $x$. \emph{Planning} (choosing future controls $u$) requires extending the generative model to the future. Introduce future states $(y', x', u)$ where primes denote future quantities, and a \emph{preference model} $\hat{p}(x')$ encoding desired future configurations. The quantity that scores a policy $u$ is the \emph{Expected Free Energy} (EFE) \cite{dacostaactive2024}:
\begin{equation}\label{eq:eng-efe}
    G(u) = \underbrace{\mathbb{E}_{q}\left[\log\frac{q(x'|u)}{\hat{p}(x')}\right]}_{\text{risk (exploitation)}} + \underbrace{\mathbb{E}_{q}\left[\mathbb{H}[p(y'|x')]\right]}_{\text{ambiguity (exploration)}}\,.
\end{equation}
Risk penalizes policies whose predicted future states $q(x'|u)$ deviate from preferred states $\hat{p}(x')$, promoting goal-directed behavior. Ambiguity penalizes policies that lead to uninformative observations, promoting information-seeking behavior. Both exploitation and exploration emerge from the single functional $G(u)$.

\subsubsection{The precise-agent assumption}\label{sec:precise-agent-assumption} The EFE \eqref{eq:eng-efe} arises from the full future VFE under a \emph{precise-agent} assumption \cite{dacostaactive2024,barpgeometric2022}. A precise agent satisfies two conditions:
\begin{itemize}
\item[\textbf{F4a}] \emph{Precise likelihood:} $p(y'|x') = \delta_{f(x')}(y')$, i.e., observations are noiseless.
\item[\textbf{F4b}] \emph{Precise policy:} $q(u|x') = \delta_{g(x')}(u)$, i.e., actions are deterministic given the state estimate.
\end{itemize}
Under F4a and F4b, a cross-term in the full future VFE evaluates to zero \cite{dacostaactive2024}:
\begin{equation}\label{eq:eng-cross-term}
    \mathbb{E}\left[\log p(y'|x') - \log q(u|x')\right] = \log 1 - \log 1 = 0\,,
\end{equation}
and the future VFE reduces exactly to the EFE \eqref{eq:eng-efe}.

\subsubsection{Macro-particles: how precision emerges from nesting}\label{sec:macro-particles} A macroscopic AIF agent assembled from $N$ nested micro-agents naturally satisfies F4a--F4b in the limit of large $N$. Each micro-agent observes $x$ through an independent sensor with noise variance $\sigma_y^2$; the aggregate observation $\bar{y} = N^{-1}\sum_i y_i$ has variance $\sigma_y^2/N$. As $N$ grows, the collective observation becomes asymptotically noiseless:
\begin{equation}\label{eq:eng-macro-precision}
    \mathrm{Var}(\bar{y} - x) = \frac{\sigma_y^2}{N} \;\xrightarrow{N\to\infty}\; 0\,,
\end{equation}
satisfying F4a. Similarly, the average action $\bar{u}$ of $N$ micro-agents with stochastic policies has variance $\sigma_u^2/N \to 0$, satisfying F4b. A biological brain is composed of $\sim 10^{11}$ neurons, each a micro-AIF agent; their collective averaging provides the effective precision that allows the organism to be described as planning by minimizing EFE \cite{fristonparcels2020,fristonpixels2024}.

\subsubsection{Quantitative illustration: VFE converges to EFE}\label{sec:vfe-converges-to-efe} Consider a collective of $N$ micro-agents, each observing a shared external state $x$ through an independent sensor: $y_i = x + \varepsilon_i$, $\varepsilon_i \sim \mathcal{N}(0,\sigma_y^2)$. The agent prefers $x^* = 5$, encoded as $\hat{p}(x') = \mathcal{N}(x' | 5,\,\sigma_\mathrm{goal}^2)$ with $\sigma_\mathrm{goal}^2 = 4$, $\sigma_y^2 = 1$. The collective VFE for a one-step policy $u$ (predicted state $\mu_x(u) = u$) evaluates to:
\begin{equation}\label{eq:eng-vfe-macro}
    F_N(u) = \underbrace{\frac{(u - x^*)^2}{2\sigma_\mathrm{goal}^2}}_{\text{risk}} + \underbrace{\frac{\sigma_y^2/N}{2\sigma_\mathrm{goal}^2}}_{\text{precision residual}} + \underbrace{\frac{1}{2}\log\frac{2\pi e\,\sigma_y^2}{N}}_{\text{ambiguity}}\,.
\end{equation}
\begin{center}
\begin{tabular}{c c c l}
\toprule
$N$ & Precision residual & Ambiguity & Policy selection governed by \\
\midrule
1   & $0.125$ & $+1.42$ & risk $+$ residual $+$ ambiguity (full VFE) \\
10  & $0.013$ & $+0.27$ & risk $+$ small corrections \\
100 & $0.001$ & $-0.88$ & risk (corrections $\ll 1$) \\
$\infty$ & $0$ & $-\infty$ (const.)${}^\dagger$ & risk only = EFE \\
\bottomrule
\end{tabular}
\end{center}
\noindent ${}^\dagger$ The ambiguity diverges equally for all policies and does not affect relative policy ranking.

As $N$ grows, the precision residual vanishes and the ambiguity becomes a policy-independent constant. Policy comparison therefore reduces to minimizing the risk alone, the EFE for a precise agent. The selected policy is then:
\begin{equation}\label{eq:eng-policy-posterior}
    q(u) \;\propto\; \exp\bigl(-G(u)\bigr)\,,
\end{equation}
a softmax over EFE values: low-EFE policies are exponentially preferred.

%---------------------------------------------------------------
\subsection{Expected Free Energy from Epistemic Priors}
%---------------------------------------------------------------

The precise-agent route to EFE relies on a physical limiting argument ($N\to\infty$). An alternative derivation, developed in \cite{vriesexpected2025,nuijtenmessage2026}, avoids this limit entirely and shows that EFE minimization is equivalent to standard VFE minimization in an \emph{augmented} generative model.

Specifically, augment the predictive model $p(y',x',u)$ and the preference prior $\hat{p}(x')$ with two \emph{epistemic priors}:
\begin{align}\label{eq:eng-epistemic-priors}
    \tilde{p}(u) &= \exp\bigl(+\mathbb{H}[q(x'|u)]\bigr)\,, \notag\\
    \tilde{p}(x') &= \exp\bigl(-\mathbb{H}[q(y'|x')]\bigr)\,,
\end{align}
where $\mathbb{H}[\cdot]$ is Shannon entropy. The prior $\tilde{p}(u)$ rewards policies that preserve uncertainty about future states, an explicit \emph{exploration} incentive. The prior $\tilde{p}(x')$ penalizes visiting external states from which observations are ambiguous, promoting \emph{information gain}.

Under the augmented model, the VFE functional
\begin{equation}\label{eq:eng-augmented-vfe}
    F[q] = \mathbb{E}_q\left[\log\frac{q(y',x',u)}{p(y',x',u)\,\hat{p}(x')\,\tilde{p}(x')\,\tilde{p}(u)}\right]
\end{equation}
evaluates to \cite{vriesexpected2025,nuijtenmessage2026}:
\begin{equation}\label{eq:eng-efe-as-vfe}
    F[q] = \underbrace{\mathbb{E}_{q(u)}\left[G(u)\right]}_{\text{expected EFE}} + \underbrace{\mathbb{E}_{q(y',x',u)}\left[\log\frac{q(y',x',u)}{p(y',x',u)}\right]}_{\text{complexity}}\,.
\end{equation}
Minimizing \eqref{eq:eng-augmented-vfe} simultaneously minimizes expected EFE and a complexity penalty that discourages overly intricate policy posteriors, intrinsically regulating computational resources.

This result is important for three reasons. First, it removes the need for the precise-agent assumption: EFE scoring of policies emerges from VFE minimization under suitable modeling commitments, not from a physical limit argument. Second, the complexity term in \eqref{eq:eng-efe-as-vfe} provides natural computational regularization: complex policy posteriors cost more free energy, favoring simpler and more efficient inference. Third, both epistemic priors have clear engineering interpretations: $\tilde{p}(u)$ is an entropy bonus (analogous to a temperature parameter in reinforcement learning softmax policies), and $\tilde{p}(x')$ is a mutual-information reward (encouraging policies that maximize information gain about external states). Crucially, both are derived from a single variational principle rather than hand-tuned.

From a signal processing perspective, incorporating epistemic priors is analogous to adding information-theoretic regularization to the inference objective. Just as $\ell_1$ regularization in compressed sensing promotes sparse solutions, epistemic priors in AIF promote information-efficient policies.

%---------------------------------------------------------------
\subsection{Reactive Message Passing: Scalable AIF in Practice}\label{sec:factor-graphs}
%---------------------------------------------------------------

The generative model \eqref{eq:eng-gen-model}, augmented with preference and epistemic priors \eqref{eq:eng-epistemic-priors}, specifies what an AIF agent must compute. The engineering question is \emph{how} to compute it efficiently under real-world constraints.

\subsubsection{Factor graphs}\label{sec:eng-factor-graphs}

The generative model factorizes into a product of local terms. Representing this factorization as a Forney-style factor graph allows VFE minimization to be decomposed into local message-passing updates \cite{winnvariational2005,dauwelsvariational2007a}. As established in Section~\ref{sec:factor-graphs}, stationary points of the Constrained Bethe Free Energy (CBFE) on the graph correspond to fixed points of belief propagation or variational message passing. Each node computes outgoing messages from incoming messages using only local factor information, with no central coordinator required.

The nested AIF structure is directly mirrored: each subgraph (sub-agent) minimizes a local CBFE contribution, and the global CBFE is the sum of local terms. This confirms that a factor graph implementing an AIF agent \emph{is} a network of nested AIF agents, and vice versa.

\subsubsection{Reactive message passing}\label{sec:reactive-message-passing} In physical environments, sensor inputs arrive asynchronously, computational budgets fluctuate, and inference deadlines vary. Standard (fixed-schedule) message passing is inadequate for these conditions. Reactive message passing \cite{bagaevrxinfer2023,bagaevreactive2023a,devriesdesign2024} addresses this through an event-driven scheduling discipline:
\begin{itemize}
    \item A node emits an updated outgoing message \emph{only when one of its incoming messages changes meaningfully}.
    \item Priority is assigned based on the magnitude of each node's contribution to the CBFE gradient: nodes that most reduce free energy are updated first.
    \item Inference can be halted at any point; the current beliefs are the best available given the messages computed so far (\emph{anytime inference}).
\end{itemize}

This architecture handles the resource constraints of physical AI agents directly:
\begin{itemize}
    \item \emph{Temporal constraints (real-time deadlines):} High-priority nodes (e.g., obstacle-avoidance factors) are processed before low-priority nodes (e.g., long-horizon planning factors). The CBFE provides a principled priority criterion.
    \item \emph{Data constraints (asynchronous sensors):} A 100~Hz IMU and a 10~Hz camera each trigger message updates on their own schedules; no global synchronization is required.
    \item \emph{Power constraints:} When energy is limited, updates to lower-priority subgraphs (e.g., learning factors) are suspended; the agent continues to operate correctly on the remaining subgraph.
\end{itemize}

\subsubsection{Scalability}\label{sec:eng-scalability} Adding a new sensor or actuator corresponds to appending a new factor node to the graph; no existing code needs modification. This plug-and-play modularity is essential for physical systems that reconfigure their sensor-actuator arrangements in the field. Multi-agent teams extend naturally: each agent maintains its own factor graph, and inter-agent communication corresponds to message passing between graphs via shared external-state variable nodes.

The RxInfer framework \cite{bagaevrxinfer2023} realizes this architecture in software: a reactive probabilistic programming environment in which the generative model is specified declaratively, and all inference computations (filtering, smoothing, planning, learning) are derived automatically as reactive message-passing rules \cite{devriesdesign2024}.

\subsubsection{Three concurrent inference streams}\label{sec:three-inference-streams} The factor graph of an AIF agent runs three concurrent message streams:
\begin{enumerate}
    \item \emph{Backward pass (perception):} messages from observation factors $p(y|x)$ toward internal states $s$ perform real-time filtering, a Kalman filter for linear-Gaussian models or a particle filter for nonlinear and non-Gaussian models.
    \item \emph{Forward pass (planning):} messages from the preference factor $\hat{p}(x')$ and epistemic priors propagate backward through dynamics factors $p(x'|u)$, computing optimal policies, functionally equivalent to a backward dynamic program.
    \item \emph{Bidirectional pass (learning):} messages flow to and from parameter factors, continuously updating model parameters, implementing online stochastic variational EM.
\end{enumerate}
In the reactive setting, these streams interleave automatically: new observations trigger perception updates, which trigger planning updates, which trigger action outputs, which trigger new observations. Perception, planning, and learning are not separate modules; they are concurrent message flows in a single reactive graph.

%---------------------------------------------------------------
\subsection{Distributed AIF: A Robot Football Team}
%---------------------------------------------------------------

We return to the robot football scenario introduced in Section~\ref{sec:abstract} to illustrate how a team of AIF agents can coordinate without centralized control.

\subsubsection{Individual player as an AIF agent}\label{sec:individual-player-aif} Each robot player $i$ ($i = 1,\ldots,K$) is an AIF agent with:
\begin{itemize}
    \item Sensory states $y_i$: camera images, LIDAR, IMU, and communication inputs from teammates.
    \item External states $x_i$: positions and velocities of ball, teammates, and opponents.
    \item Control states $u_i$: wheel commands, kick parameters, gaze direction.
    \item Internal states $s_i$: parameters of the recognition density $q_{s_i}(x_i)$, encoding the player's world model.
    \item Preference model $\hat{p}_i(x_i)$: role-specific goal distribution: for an attacker, ball at the opponent's goal; for a goalkeeper, ball outside the penalty area; for a midfielder, maintaining possession in advantageous positions.
\end{itemize}
Each player minimizes its individual EFE $G_i(u_i)$ \eqref{eq:eng-efe}: the risk term drives role-specific goal achievement (moving toward the ball, intercepting passes, covering space), while the ambiguity term promotes information-seeking actions such as scanning uncertain field regions or requesting positional updates from teammates.

\subsubsection{Team as a nested AIF agent}\label{sec:team-nested-aif} The $K$-player team satisfies conditions E1--E3:
\begin{itemize}
    \item \emph{E1}: Players interact through the shared environment (ball, field, opponents); no player's internal states $s_i$ directly drive another's internal computation. The collective blanket property follows from F3 and E1.
    \item \emph{E2}: Individual perception-action cycles run at ca.\ 10--100~ms; team-level tactical adjustments evolve over 1--10~s, satisfying the adiabatic condition.
    \item \emph{E3}: Collective team dynamics feed back onto individual players through role assignments and tactical instructions, ensuring feedback closure.
\end{itemize}
Under E1--E3, the team is itself an AIF agent at a coarser spatiotemporal scale. Its collective VFE is:
\begin{equation}\label{eq:eng-team-vfe}
    F_\mathrm{team} = \sum_{i=1}^{K} F_i + \sum_{(i,j)\in\mathcal{E}} F_{ij}\,,
\end{equation}
where $F_{ij}$ captures information coupling between players $i$ and $j$ who share a common external state $x$ (e.g., two players competing for the same ball). The team's collective preference model $\hat{p}(x_\mathrm{team})$ encodes the team objective: winning the match.

\subsubsection{Emergent coordination via reactive message passing}\label{sec:emergent-coordination} Team coordination is not explicitly programmed. When player $A$ updates its belief $q_{s_A}(x)$ about the ball's position, this update propagates via the coupling factors $F_{AB}$ to player $B$'s factor graph, reshaping $B$'s policy posterior without any explicit coordination protocol. Tactical patterns (pressing, covering space, switching play) emerge from belief propagation across the inter-agent factor graph.

The architecture handles real-world robustness naturally: if a player loses communication (E1 temporarily broken), it falls back to its individual VFE; if a player's sensors degrade, inference slows but remains valid; if the opposing team changes tactics, the online learning stream continuously updates generative model parameters. In each case, the CBFE provides a principled criterion for degraded-mode operation, a property that explicit planning algorithms lack.

This robot football example illustrates the broader promise of distributed AIF for physical AI: scalable, adaptive, and robust collective behavior emerges from local VFE minimization, without centralized planning or explicit inter-agent protocol design. The mathematical framework underlying the Mbapp\'e-level physical intelligence we aspire to (and that the FEP claims characterizes biological systems) is precisely this hierarchy of nested VFE-minimizing agents, realized through reactive message passing on factor graphs.

%---------------------------------------------------------------


==> sections/unused/nested-aif.tex <==
\section{Nested Active Inference in Factor-Graph Form}
\label{sec:nested-aif-fg}

In the previous sections, we formulated active inference as constrained variational inference, implemented as Constrained Bethe Free Energy (CBFE) minimization on a Forney-style factor graph. We now make explicit that \emph{the nested structure of AIF agents follows directly from the compositional properties of factor graphs and the scale-invariance of CBFE minimization}.

\subsection*{A Single AIF Agent as a Factor Graph}

Recall that an AIF agent is specified by a generative model
\begin{equation}
    p(s,x,u,y)
    =
    p(s | x)\,
    p(x | u)\,
    p(u | y)\,
    p(y),
\end{equation}
with Markov blanket partition $(s,u)$ separating internal states $y$ from external states $x$:
\begin{equation}
    y \perp x | (s,u).
\end{equation}

In factor-graph form, this model decomposes into local factors
\[
f_1(s,x),\quad
f_2(x,u),\quad
f_3(u,y),\quad
f_4(y).
\]

CBFE minimization corresponds to solving
\begin{equation}
    q^\star = \arg\min_{q \in \mathcal{Q}} F_{\text{CBFE}}[q],
\end{equation}
where $q$ factorizes according to the graph structure and the constraints in $\mathcal{Q}$ encode local marginal consistency.

As shown earlier, stationary points of $F_{\text{CBFE}}$ correspond to fixed points of message passing. Hence, a single AIF agent is realized as a self-consistent set of local inference updates on a structured factor graph.

\subsection*{Composition of Multiple AIF Agents}

Now consider $N$ interacting AIF agents indexed by $i=1,\dots,N$, each with states $(s_i,x_i,u_i,y_i)$ and local generative model
\[
p_i(s_i,x_i,u_i,y_i).
\]

Suppose their interaction is mediated through shared variables or coupling factors:
\begin{equation}
    p(\{s_i,x_i,u_i,y_i\}_{i=1}^N)
    =
    \prod_{i=1}^N p_i(s_i,x_i,u_i,y_i)
    \;
    \prod_{(i,j)\in\mathcal{E}} \psi_{ij}(u_i,x_j),
\end{equation}
where $\psi_{ij}$ encodes inter-agent coupling.

This defines a larger factor graph obtained by \emph{gluing} the individual graphs along shared edges. Crucially, factor graphs are closed under composition: the union of locally consistent factorizations is again a valid global factorization.

\subsection*{Emergence of a Higher-Level Markov Blanket}

Define coarse-grained states
\begin{align}
    x^{(2)} &= \Phi_x(\{x_i\}), \\
    s^{(2)} &= \Phi_s(\{s_i\}), \\
    u^{(2)} &= \Phi_u(\{u_i\}), \\
    y^{(2)} &= \Phi_y(\{y_i\}),
\end{align}
where the mappings $\Phi_\cdot$ define sufficient statistics at the higher scale.

If the aggregate system admits a Markov blanket partition
\begin{equation}
    y^{(2)} \perp x^{(2)} | (s^{(2)},u^{(2)}),
\end{equation}
and if the joint density reaches a nonequilibrium steady state (NESS), then by the FEP lemma (cf.\ \cite[Sec.~8]{fristonfree2019}) the higher-level autonomous states minimize a corresponding free energy functional.

In factor-graph terms, this corresponds to marginalizing over internal fine-scale variables:
\begin{equation}
    p^{(2)}(s^{(2)},x^{(2)},u^{(2)},y^{(2)})
    =
    \int
    p(\{s_i,x_i,u_i,y_i\})
    \,\delta(\Phi - \text{constraints})
    \,d\{s_i,x_i,u_i,y_i\}.
\end{equation}

Because Bethe free energy is additive over factors,
\begin{equation}
    F_{\text{CBFE}}^{\text{tot}}
    =
    \sum_{i=1}^N F_{\text{CBFE}}^{(i)}
    +
    \sum_{(i,j)\in\mathcal{E}} F_{\psi_{ij}},
\end{equation}
its stationary points are preserved under marginalization whenever consistency constraints remain satisfied.

Thus, if each lower-level agent satisfies local CBFE optimality and the coupling preserves marginal consistency, then the aggregate system satisfies
\begin{equation}
    \nabla F_{\text{CBFE}}^{(2)} = 0.
\end{equation}

\textbf{Hence, CBFE minimization is closed under graph composition and marginalization.}

\subsection*{Renormalization Interpretation}

Coarse graining corresponds to contracting subgraphs into super-nodes. The renormalization group studies how objective functionals transform under such contractions.

If the functional form of the objective is preserved, it is a renormalization fixed point.

Because:

\begin{enumerate}
    \item factor graphs compose by union,
    \item CBFE is additive over factors,
    \item stationary points correspond to local message-passing fixed points,
\end{enumerate}

CBFE minimization is invariant under graph contraction. In this precise sense, VFE minimization is a fixed point of coarse graining.

This mirrors the scale-free arguments in \cite{fristonpixels2024} and the recursive blanket construction in \cite{fristonparcels2020}.

\subsection*{Evolution as Bottom-Up Graph Construction}

Evolution can be interpreted as iterated graph composition:

\begin{itemize}
    \item Local self-organizing subsystems (cells) correspond to stable CBFE minima.
    \item Stable subsystems couple through interaction factors.
    \item Coarse-grained aggregates that admit Markov blanket partitions persist.
\end{itemize}

Only configurations that maintain NESS densities and local marginal consistency survive selection. Over evolutionary time, this produces hierarchical factor graphs whose subgraphs are themselves AIF agents.

Therefore, a biological organism is not a single monolithic inference machine; it is a hierarchy of nested CBFE-minimizing subgraphs.

\subsection*{Conclusion}

An AIF agent is a nested AIF agent because:

\begin{enumerate}
    \item A single agent corresponds to CBFE minimization on a factor graph.
    \item Factor graphs are closed under composition and marginalization.
    \item CBFE stationary points are preserved under graph contraction.
    \item Evolution builds higher-level agents from lower-level CBFE-stable subsystems.
\end{enumerate}

Thus, nestedness is not metaphorical; it is a structural consequence of the compositional algebra of factor graphs and the scale-invariance of constrained free-energy minimization.
%---------------------------------------------------------------

